Computational Flash Photography through Intrinsics

Flash is an essential tool as it often serves as the sole controllable light source in everyday photography. However, the use of flash is a binary decision at the time a photograph is captured with limited control over its characteristics such as strength or color. In this work, we study the computational control of the flash light in photographs taken with or without flash. We present a physically motivated intrinsic formulation for flash photograph formation and develop flash decomposition and generation methods for flash and no-flash photographs, respectively. We demonstrate that our intrinsic formulation outperforms alternatives in the literature and allows us to computationally control flash in in-the-wild images.

==> imagetex/IAN.tex <==
\begin{figure*} \centering


\includegraphics[width=0.8\linewidth]{images/ian.jpg}
\caption{Comparison between our method to IAN~\cite{zhu2022ian} in decomposition (row one to three) and generation task (row four to six). Row six is not from our test set. 
}
\label{fig:IAN_dec}
\end{figure*}

==> imagetex/IAN_comp.tex <==
\begin{figure*}
\includegraphics[width=1\linewidth]{images/IAN.jpg}
\caption{As observed in rows one and two, the IAN estimates lack visual quality in the portrait images. In addition,we saw that in some cases  the estimates do not completely relight the sceneries as seen from the last row. \sepideh{probably need to make this figure smaller or put it in the supplementary.}
}
\label{fig:IAN_comp}
\end{figure*}




==> imagetex/ambientPor.tex <==
\begin{figure}\centering
\includegraphics[width=1\linewidth]{images/colorbalancedportrait.jpg}

\caption[Color balancing ambient illumination in DPD]{
 The ambient color of the foregrounds from the DPD~\cite{deepflash} is matched with the ambient color of backgrounds from FAID~\cite{flashambient} by matching the ratio between the ambient and flash images.
}
\label{fig:ambientPor}
\end{figure}

==> imagetex/atod65.tex <==
\begin{figure}[H] \centering
\includegraphics[width=1\linewidth]{images/atod65.jpg}
\caption[Chromatic adaptation]{The images in illuminant A in FAID~\cite{flashambient} are converted to illuminant D65 through chromaticity adaptation.}
\label{fig:atod65}
\end{figure}

==> imagetex/badFlash.tex <==
\begin{figure*}\centering
\includegraphics[width=1\linewidth]{images/bad_flash.jpg}
\caption[removed flash illuminations]{Photos with a dim flash illumination are not included in the database. This occurs when subjects are too far away from the camera}
\label{fig:bad_flash}
\end{figure*}

==> imagetex/decomposition_abl.tex <==
\begin{figure}
\includegraphics[width=1\linewidth]{images/decompose_abl.jpg}
\caption{Ablation on decomposition
}
\label{fig:decompose_abl}
\end{figure}




==> imagetex/deepFlash.tex <==
\begin{figure*} \centering
\negvspace
\negvspace


\includegraphics[width=0.8\linewidth]{images/deepflash.jpg}
\caption[Deep Flash]{Comparison between our method to Deep Flash~\cite{deepflash}'s in the decomposition task. The last row is not from the test set. 
}
\negvspace
\negvspace


\label{fig:deepflash}
\end{figure*}

==> imagetex/flashPor.tex <==
\begin{figure}\centering
\includegraphics[width=1\linewidth]{images/flash_color.jpg}

\caption[Color balancing flash illumination in DPD]{
 The flash color of the people in the DeepFlash Portrait dataset~\cite{deepflash} is matched with the flash color of background images.
}
\label{fig:flashPor}
\end{figure}

==> imagetex/flash_edit.tex <==
\begin{figure*}
\includegraphics[width=\linewidth]{images/flash_edit.jpg}
\caption{
The separate flash and ambient shadings we estimate for a given flash photograph can be edited separately to render the same scene under varying illuminations.
}
\label{fig:appSpectrum}
\end{figure*}

==> imagetex/generation_abl.tex <==
\begin{figure}
\includegraphics[width=1\linewidth]{images/generation_abl.jpg}
\caption{Ablation on generation
}
\label{fig:decompose_abl}
\end{figure}




==> imagetex/highres_arc.tex <==
\begin{figure}
\includegraphics[width=\linewidth]{images/highres.jpg}

\caption[High Resolution and boosting Network]{The ratio between the high resolution flash photo and estimated low resolution ambient from the Decomposition network is computed and given to the high resolution network alongside the input flash photograph. The high resolution ratio estimation gets the details from the flash photo and the illumination from the low resolution ratio. By multiplying the flash photograph by the estimated high resolution ratio, the final high resolution ambient illumination is generated. 
}
\label{fig:highres}
\end{figure}




==> imagetex/highres_results.tex <==
\begin{figure}[H]\centering
\includegraphics[width=\linewidth]{images/highres_sh.jpg}

\caption{ 
The high resolution method is done as a post-processing step for both generation (first row) and decomposition tasks (second and third row).
}
\label{fig:highres_sh}
\end{figure}

==> imagetex/multiExample.tex <==
\begin{figure}\centering
\includegraphics[width=1\linewidth]{images/multi_examples.jpg}
\caption[Multi Illumination dataset flash and ambient]{The Multi-Illumination Dataset features a variety flash-illuminated captures for the same scene. Each scene has one capture with direct flash illumination. The other captures utilize a bounce-flash and can therefore be used as indirect ambient illuminations. This provides 20 different ambient illuminations to be used as augmentation}
\label{fig:multi_examples}
\end{figure}

==> imagetex/normalizedAmbient.tex <==
\begin{figure}\centering
\includegraphics[width=\linewidth]{images/brightness_normalized.jpg}

\caption[Ambient illumination brightness normalization]{
The brightness of ambient illumination is normalised relative to the L channel in CIELAB, resulting in images with approximately the same level of brightness throughout the dataset.
}
\label{fig:normalizedAmbient}
\end{figure}

==> imagetex/oiddr.tex <==
\begin{figure*} \centering
\includegraphics[width=1\linewidth]{images/oiddr.jpg}
\caption[OIDDR]{ Comparison between our method to OIDDR~\cite{Yazdani2021PhysicallyID}'s in generation task (row one to three) and decomposition task (row four and five) for both the shading and final illumination. Row three and five are not from our test set.
}
\label{fig:oiddr}
\end{figure*}

==> imagetex/pix2pix_faid.tex <==
\begin{figure*} \centering
\includegraphics[width=\linewidth]{images/faid_pix2pixhd.jpg}
\caption{Comparison between our method to Pix2PixHD~\cite{pix2pixHD} and FAID~\cite{flashambient} in decomposition (row one and three) and generation task (row two and four). Row three and four are not from the test set and we do not have the ground truth for them.
}
\label{fig:faid_pix2pixHD}
\end{figure*}

==> imagetex/portraitExample.tex <==
\begin{figure}\centering
\includegraphics[width=1\linewidth]{images/portrait_example.jpg}
\caption[Portrait dataset creation]{
The DeepFlash Portrait Dataset~\cite{deepflash} provides photographs taken in front of a green screen. We extract the foreground by  generating a trimap and applying standard matting techniques. These extracted foregrounds are color balanced with respect to the background from FAID and composited}
\label{fig:portrait_example}
\end{figure}


==> imagetex/teaser.tex <==

\begin{figure*}
% \centering
\includegraphics[width=\linewidth]{images/teaser.png}
\caption{
We address two aspects of computational flash photography
  \label{fig:teaser}
}
\end{figure*}


==> imagetex/temps.tex <==
\begin{figure*} %\centering
\includegraphics[width=1\linewidth]{images/temps.jpg}

\caption[Different color temperatures]{
Chromatic adjustment allows for a shift in the white-balanced image's temperature. The temperature goes from warm temperature of 2700 Kelvin to cold temperature of 9300 Kelvin.
}
\label{fig:difftemps}
\end{figure*}

==> imagetex/whiteBalance.tex <==
\begin{figure} \centering
\includegraphics[width=1\linewidth]{images/whitebalance.jpg}
\caption[White balancing the ambient illumination]{The ambient illumination can have various colors while flash illumination is always white. We white balance the ambient illumination with respect to the flash illumination.
}
\label{fig:whitebalance}
\end{figure}


==> tex/5-highres.tex <==
\input{imagetex/highres_arc}

We train our generation and decomposition networks at the resolution of $256 \times 256$ due to GPU memory constraints. 
In order to apply our results to high-resolution input, we implement a guided super-resolution framework. 
To generate high-resolution flash decomposition, Aksoy et al.~\cite{flashambient} make use of \emph{ratio images} that relate the input/output pairs. 
While Aksoy et al. use a simple edge-aware filtering~\cite{domainTransform} in high-resolution, we adopt a data-driven methodology.
We train two separate networks for the decomposition and generation tasks. 
We will adopt the variables for the decomposition task in our formulation below for clarity without loss of generality.
An overview of our setup is shown in Fig.~\ref{fig:highres}.

\paragraph{Input/Output Formulation}
The original RGB image is provided to the network together with the low-resolution ratio image that is defined as:
%
\begin{equation}
    \mathcal{R}_{LR} = \frac{2(\hat{A}+1)}{3(P+1)} - \frac{1}{3}.
\end{equation}
%
We compute $\mathcal{R}_{LR}$ at size $256 \times 256$ and upscale it to the original input resolution before feeding it to the network. 
This definition was proposed in \cite{flashambient} to restrict the ratio image in $[0,1]$. 

We define the output of our network as the high-resolution ratio image $\mathcal{R}_{HR}$, which can be used to compute the final high-resolution output:
%
\begin{equation}
    \hat{A}_{HR} = {(3\mathcal{R}_{HR}+1)(P+1)}/{2}-1.  
    \label{eq:ratioInverse}
\end{equation}
%

\paragraph{Losses and Network Structure}
We use the $L_1$ and the multi-scale gradient losses defined in Eqs.~\ref{eq:L1} and \ref{eq:gradLoss} on the output image and backpropagate it through Eq.~\ref{eq:ratioInverse}:
\begin{equation}
    \mathcal{L}_{HR} = \mathcal{L}_{1,A} + 
                    0.5 \mathcal{L}_{g,A}.
\end{equation}

As the generator, we employed an 8-layer u-net\cite{unet} based encoder decoder network, with the PatchGAN~\cite{pix2pix} as the critic network, which discriminates the images at the scale of $70\times 70$ patches. We used an initial learning rate of 0.0002 and train for 100 epochs with the initial learning rate and 100 epochs with a linearly decreasing the learning rate. The high resolution estimation size is set to 1024 by 1024 pixels.



==> tex/8-applications.tex <==
One significant advantage of the intrinsic model is its ability to generate shadings and ambient shading color. Figure~\ref{fig:qual_dec} shows two decomposition examples with their shadings. Having the shadings also make editing the flash and ambient illuminations easier.  Figure~\ref{fig:qual_dec_comp} shows altering estimated ambient shading color in the input flash photograph. In figure~\ref{qual_gen}, we generated the flash shading and also were able to edit it to make it look more strong. 

